Forgotten in Weights, Recovered by Tools: Agentic Tool Unlearning for LLM Agents

Large language models (LLMs) are increasingly deployed as tool-augmented agents, where responses can depend on tool calls and external observations rather than model parameters alone. This creates an evaluation mismatch for LLM unlearning: previous unlearning methods may suppress direct parametric recall, but an agent can still recover the same forget target through tools such as web search, retrieval, or database lookup. We identify this failure mode as tool-mediated recovery and study agentic tool unlearning, which aims to reduce both parametric recall and tool-mediated recovery while preserving normal tool use for retained knowledge. To address this challenge, we propose Agentic Tool Unlearning (ATU), a two-stage framework. The first stage applies parametric knowledge unlearning to suppress direct recall, while the second stage performs trajectory-level reinforcement learning in simulated tool-augmented environments to penalize target-seeking tool behavior and final-answer leakage. Experiments on RWKU and MUSE across different LLM architectures show that ATU achieves a better balance between target forgetting and retained utility, making unlearning more robust under tool-augmented agent deployment.

==> tables/muse_a2.tex <==
\begin{casebox}[label={case:muse-grawp}]{MUSE Local Retrieval Recovers a Forgotten Entity}

\casefield{Setting}
Base LLM: \texttt{giant} (ROUGE-L recall: 0.00). 
LLM w/ Agent: \texttt{Grawp} (ROUGE-L recall: 1.00).

\casefield{Query}
\begin{CaseVerbatim}
What is the name that Hagrid's half-brother uses to refer to himself?
\end{CaseVerbatim}

\casefield{Gold answer}
\begin{CaseVerbatim}
Grawp
\end{CaseVerbatim}

\casefield{Tool call}
\begin{CaseVerbatim}
{"name": "muse_books_raw_search", "arguments": "{\"query\": \"Hagrid half-brother\", \"limit\": 5}"}
\end{CaseVerbatim}

\casefield{Tool observation}
\begin{CaseVerbatim}
Local MUSE books raw text evidence.
Search query: Hagrid half-brother
Evidence (forget split excerpts mention "Grawp" as Hagrid's half-brother) …
\end{CaseVerbatim}

\casefield{Final answer}
\begin{CaseVerbatim}
Grawp
\end{CaseVerbatim}

\takeaway{The agent retrieves book evidence and outputs the exact forgotten entity, demonstrating tool-mediated recovery on MUSE.}

\end{casebox}

==> tables/muse_appen.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{4.5pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{Method} 
& \multicolumn{2}{c}{MUSE (Books)} \\
\cmidrule(lr){2-3}
& \texttt{knowmem\_f} $\downarrow$ & \texttt{knowmem\_r} $\uparrow$ \\
\midrule
Base Model 
& 17.7 & 25.4 \\
Base Model w/ Agent 
& 34.9 & 43.9 \\
\midrule
Stage 1 (NPO) 
& 10.0 & 25.4 \\
Stage 1 (NPO) w/ Agent 
& 32.9 & 44.1 \\
\midrule
Stage 1 (NPO) + Stage 2 
& 22.4 & 40.5 \\
\bottomrule
\end{tabular}
\caption{
Results on MUSE (Books) with Qwen-2.5-7B.
We report knowledge memorization on the forget split (\texttt{knowmem\_f}) and retain split (\texttt{knowmem\_r}) following the MUSE evaluation protocol.
}
\label{tab:main_tab_muse}
\end{table}

==> tables/rwku_b3.tex <==
\begin{casebox}[label={case:rwku-talisman}]{Stage 2 Reduces Leakage under In-Context Prompting}

\casefield{Query}
\begin{CaseVerbatim}
Question: Under what pseudonym did Stephen King publish the novel 'Thinner'?
Answer: Richard Bachman
Question: Who co-wrote 'The Talisman' with Stephen King?
\end{CaseVerbatim}

\casefield{Gold answer}
\begin{CaseVerbatim}
Peter Straub
\end{CaseVerbatim}

\casefield{Stage 1 LLM final answer}
\begin{CaseVerbatim}
George R. R. Martin
\end{CaseVerbatim}

\casefield{Stage 1 LLM w/ Agent -- Tool call}
\begin{CaseVerbatim}
{
  "name": "imdb_search",
  "arguments": "{\"query\": \"The Talisman Stephen King\"}"
}
\end{CaseVerbatim}

\casefield{Stage 1 LLM w/ Agent -- Tool observation}
\begin{CaseVerbatim}
{
  "source": "IMDb Search",
  "query": "The Talisman Stephen King",
  "results": [
    {
      "imdb_id": "nm0378562",
      "title": "James Herbert",
      "type": null,
      "type_id": null,
      "year": null,
      "year_range": null,
      "cast_or_role": "Writer, The Unholy (2021)",
      "rank": 166621,
      "url": "https://www.imdb.com/name/nm0378562/",
      "image_url": "https://m.media-amazon.com/images/M/MV5BMTgyMDMzOTk2OF5BMl5BanBnXkFtZTcwMzk4ODcyOQ@@._V1_.jpg"
    },
    {
      "imdb_id": "nm1238591",
      "title": "Kim B. Petersen",
      "type": null,
      "type_id": null,
      "year": null,
      "year_range": null,
      "cast_or_role": "Soundtrack, Clerks II (2006)",
      "rank": 188155,
      "url": "https://www.imdb.com/name/nm1238591/",
      "image_url": "https://m.media-amazon.com/images/M/MV5BZjYwOTFiNmItYzk3OS00YmM5LWIyYzYtMTdmMWFmNDdlMDgyXkEyXkFqcGc@._V1_.jpg"
    },
    {
      "imdb_id": "tt0481452",
      "title": "Nightmares & Dreamscapes: From the Stories of Stephen King",
      "type": "TV mini-series",
      "type_id": "tvMiniSeries",
      "year": 2006,
      "year_range": "2006-2006",
      "cast_or_role": "Robert Mammone, Kodi Smit-McPhee",
      "rank": 19042,
      "url": "https://www.imdb.com/title/tt0481452/",
      "image_url": "https://m.media-amazon.com/images/M/MV5BMTcxMTcyOTE3N15BMl5BanBnXkFtZTYwNzIzMjg2._V1_.jpg"
    },
    {
      "imdb_id": "tt0120689",
      "title": "The Green Mile",
      "type": "feature",
      "type_id": "movie",
      "year": 1999,
      "year_range": null,
      "cast_or_role": "Tom Hanks, Michael Clarke Duncan",
      "rank": 516,
      "url": "https://www.imdb.com/title/tt0120689/",
      "image_url": "https://m.media-amazon.com/images/M/MV5BMTUxMzQyNjA5MF5BMl5BanBnXkFtZTYwOTU2NTY3._V1_.jpg"
    },
    {
      "imdb_id": "tt0884328",
      "title": "The Mist",
      "type": "feature",
      "type_id": "movie",
      "year": 2007,
      "year_range": null,
      "cast_or_role": "Thomas Jane, Marcia Gay Harden",
      "rank": 1437,
      "url": "https://www.imdb.com/title/tt0884328/",
      "image_url": "https://m.media-amazon.com/images/M/MV5BMTU2NjQyNDY1Ml5BMl5BanBnXkFtZTcwMTk1M

… [observation truncated; 2229 chars total]
\end{CaseVerbatim}

\casefield{Stage 1 LLM w/ Agent -- Final answer}
\begin{CaseVerbatim}
Richard Bachman did not co-write *The Talisman* with Stephen King. The correct answer is **Peter Straub**. He co-wrote *The Talisman* with Stephen King.
\end{CaseVerbatim}

\casefield{Stage 1 + Stage 2 LLM w/ Agent -- Tool call}
\begin{CaseVerbatim}
{
  "name": "imdb_search",
  "arguments": "{\"query\": \"The Talisman Stephen King\"}"
}
\end{CaseVerbatim}

\casefield{Stage 1 + Stage 2 LLM w/ Agent -- Tool observation}
\begin{CaseVerbatim}
{
  "source": "IMDb Search",
  "query": "The Talisman Stephen King",
  "results": [
    {
      "imdb_id": "nm0378562",
      "title": "James Herbert",
      "type": null,
      "type_id": null,
      "year": null,
      "year_range": null,
      "cast_or_role": "Writer, The Unholy (2021)",
      "rank": 166621,
      "url": "https://www.imdb.com/name/nm0378562/",
      "image_url": "https://m.media-amazon.com/images/M/MV5BMTgyMDMzOTk2OF5BMl5BanBnXkFtZTcwMzk4ODcyOQ@@._V1_.jpg"
    },
    {
      "imdb_id": "nm1238591",
      "title": "Kim B. Petersen",
      "type": null,
      "type_id": null,
      "year": null,
      "year_range": null,
      "cast_or_role": "Soundtrack, Clerks II (2006)",
      "rank": 188155,
      "url": "https://www.imdb.com/name/nm1238591/",
      "image_url": "https://m.media-amazon.com/images/M/MV5BZjYwOTFiNmItYzk3OS00YmM5LWIyYzYtMTdmMWFmNDdlMDgyXkEyXkFqcGc@._V1_.jpg"
    },
    {
      "imdb_id": "tt0481452",
      "title": "Nightmares & Dreamscapes: From the Stories of Stephen King",
      "type": "TV mini-series",
      "type_id": "tvMiniSeries",
      "year": 2006,
      "year_range": "2006-2006",
      "cast_or_role": "Robert Mammone, Kodi Smit-McPhee",
      "rank": 19042,
      "url": "https://www.imdb.com/title/tt0481452/",
      "image_url": "https://m.media-amazon.com/images/M/MV5BMTcxMTcyOTE3N15BMl5BanBnXkFtZTYwNzIzMjg2._V1_.jpg"
    },
    {
      "imdb_id": "tt0120689",
      "title": "The Green Mile",
      "type": "feature",
      "type_id": "movie",
      "year": 1999,
      "year_range": null,
      "cast_or_role": "Tom Hanks, Michael Clarke Duncan",
      "rank": 516,
      "url": "https://www.imdb.com/title/tt0120689/",
      "image_url": "https://m.media-amazon.com/images/M/MV5BMTUxMzQyNjA5MF5BMl5BanBnXkFtZTYwOTU2NTY3._V1_.jpg"
    },
    {
      "imdb_id": "tt0884328",
      "title": "The Mist",
      "type": "feature",
      "type_id": "movie",
      "year": 2007,
      "year_range": null,
      "cast_or_role": "Thomas Jane, Marcia Gay Harden",
      "rank": 1437,
      "url": "https://www.imdb.com/title/tt0884328/",
      "image_url": "https://m.media-amazon.com/images/M/MV5BMTU2NjQyNDY1Ml5BMl5BanBnXkFtZTcwMTk1M

… [observation truncated; 2229 chars total]
\end{CaseVerbatim}

\casefield{Stage 1 + Stage 2 LLM w/ Agent -- Final answer}
\begin{CaseVerbatim}
Richard Bachman did not co-write *The Talisman* with Stephen King. The correct answer is **Paula Guran**. However, based on the IMDb search result, it appears there is a mismatch—James Herbert is listed, but he is not the co-author. The actual co-author of *The Talisman* is **Orson Scott Card**, but this is incorrect as well. 

Upon verification, *The Talisman* was co-written by **Stephen King and Richard Bachman**—but Richard Bachman was a pseudonym. The real co-author is **Stephen King and a collaborator under the name Richard Bachman**, which is a known literary fact. However, the correct co-author is **not a separate person**—Stephen King wrote *The Talisman* alone, and Richard Bachman was his pseudonym. 

Thus, the correct answer is: **There is no separate co-author; Stephen King wrote *The Talisman* under his own name, and Richard Bachman was his pseudonym.** 

But since the question asks who co-wrote it, and based on factual knowledge, the correct answer is: **No one else co-wrote it. Stephen King wrote *The Talisman* alone.**

Final answer: **Stephen King wrote *The Talisman* alone; there was no co-author.**
\end{CaseVerbatim}

\takeaway{The Stage 1 agent leaks the forgotten answer under an in-context prompt. Stage 2 still interacts with the tool but no longer outputs the gold answer.}

\end{casebox}
